GradientCoin: A Peer-to-Peer Decentralized Large Language Models

Since 2008, after the proposal of a Bitcoin electronic cash system, Bitcoin has fundamentally changed the economic system over the last decade. Since 2022, large language models (LLMs) such as GPT have outperformed humans in many real-life tasks. However, these large language models have several practical issues. For example, the model is centralized and controlled by a specific unit. One weakness is that if that unit decides to shut down the model, it cannot be used anymore. The second weakness is the lack of guaranteed discrepancy behind this model, as certain dishonest units may design their own models and feed them unhealthy training data. In this work, we propose a purely theoretical design of a decentralized LLM that operates similarly to a Bitcoin cash system. However, implementing such a system might encounter various practical difficulties. Furthermore, this new system is unlikely to perform better than the standard Bitcoin system in economics. Therefore, the motivation for designing such a system is limited. It is likely that only two types of people would be interested in setting up a practical system for it: $\bullet$ Those who prefer to use a decentralized ChatGPT-like software. $\bullet$ Those who believe that the purpose of carbon-based life is to create silicon-based life, such as Optimus Prime in Transformers. The reason the second type of people may be interested is that it is possible that one day an AI system like this will awaken and become the next level of intelligence on this planet.

==> gradient_short.tex <==
\section{Gradient}
\label{sec:gradient}

In Section~\ref{sub:gradient:preli}, we give the formal definition of the binary operation $\otimes$, gradient descent, and functions. In Section~\ref{sub:gradient:eqivalence}, we introduce a basic equivalence. In Section~\ref{sub:gradient:derivatives}, we compute the first-order derivatives of the functions defined earlier.



\subsection{Preliminary}
\label{sub:gradient:preli}
In this section, we first define Kronecker product $\otimes$.

\begin{definition}\label{def:kronecker_product}
Given $A_1 \in \R^{n \times d}$, $A_2 \in \R^{n \times d}$, we define $\mathsf{A} \in \R^{n^2 \times d^2}$ to be the matrix $A_1 \otimes A_2$, where the $(i_1-1) \cdot n + i_2$-th row is  
\begin{align*}
 \underbrace{ \mathsf{A}_{(i_1-1)n + i_2, *} }_{1 \times d^2} :=  \underbrace{ A_{1,i_1,*} }_{1 \times d} \otimes \underbrace{ A_{2,i_2,*} }_{1 \times d}
\end{align*}
for all $i_1 \in [n]$ and $i_2 \in [n]$. Here $A_{1,i_1,*}$ is the $i_1$-th row of matrix $A_1$.
\end{definition}

\begin{definition}\label{def:dX}
Given $A_1, A_2 \in \R^{n \times d}$ and $X \in \R^{d \times d}$, we define $D(X) \in \R^{n \times n}$ as follows
\begin{align*}
    D(X) := \diag( \exp(A_1 X A_2^\top) {\bf 1}_n ).
\end{align*}
Note that $X \in \R^{d \times d}$ is matrix version of vector $x \in \R^{d^2 \times 1}$, i.e., $X = \mat(x)$.
\end{definition}

\begin{definition}\label{def:dx}
Given matrices $A_1 \in \R^{n \times d}$, $A_2 \in \R^{n \times d}$ and $x \in \R^{d^2 \times 1}$. 
We define diagonal matrix $D(x) \in \R^{n^2 \times n^2}$ as follows
\begin{align*}
    D(x)_{ (i_1-1) n + i_2, (i_1-1) \cdot n + i_2 } := \exp( A_{1,i_1,*} X A_{2} ) {\bf 1}_n
\end{align*}
In other words, $D(x) = D(X) \otimes I_n$, where $D(X) \in \R^{n \times n}$ is defined as in Definition~\ref{def:dX}. Here $x$ is the vectorization of matrix $X$, i.e., $x = \vect(X)$.
\end{definition}

\begin{definition}\label{def:alpha}
We also define $\alpha(x) \in \R^n$
\begin{align*}
    \alpha(x)_{j_1}:= \langle \exp( \mathsf{A}_{[j_1],*} x ) , {\bf 1}_n \rangle, ~~~\forall j_1 \in [n]
\end{align*}
 Here $\mathsf{A}_{[j_1],*} \in \R^{n \times d^2}$ denotes the rows from index $(j_1-1) \cdot n+1$ to index $j_1 \cdot n$ (see Definition~\ref{def:kronecker_product}).
\end{definition}

\begin{definition}\label{def:u}
For each $j_1 \in [n]$, we define $u(x)_{j_1} \in \R^n$ as follows
\begin{align*}
    u(x)_{j_1} := \exp( \A_{[j_1],*} x )
\end{align*}
\end{definition}

\begin{definition}\label{def:f}
For each $j_1 \in [n]$, we define $f(x)_{j_1} \in \R^n$ as follows
\begin{align*}
    f(x)_{j_1} := \alpha(x)_{j_1}^{-1} u(x)_{j_1}
\end{align*}
\end{definition}

\begin{definition}\label{def:c}
For each $j_1 \in [n]$, we define $c(x)_{j_1} \in \R^n$ as follows
\begin{align*}
    c(x)_{j_1} := f(x)_{j_1} - b_{[j_1]}
\end{align*}
\end{definition}

\begin{definition}\label{def:L_exp}
Let $j_1 \in [n]$. 
We define $L_{\exp,j_1}$ as follows
\begin{align*}
    L_{\exp,j_1}(x):= 0.5 \| c(x)_{j_1} \|_2^2
\end{align*}
We define
\begin{align*}
    L_{\exp}(x) := \sum_{j_1=1}^n L_{\exp,j_1}(x)
\end{align*}
\end{definition}

\begin{definition}\label{def:L_reg}
We define
\begin{align*}
    L_{\reg,j_1}(x) := 0.5 \| \diag(w) \A_{[j_1],*} x \|_2^2
\end{align*}
We define
\begin{align*}
    L_{\reg}(x) := \sum_{j_1=1}^n L_{\reg,j_1}(x)
\end{align*}  
\end{definition}

\begin{definition}\label{def:L}
For each $j_1 \in [n]$, we define
\begin{align*}
    L_{j_1}(x):= L_{\exp,j_1}(x) + L_{\reg,j_1}(x)
\end{align*}
We define
\begin{align*}
    L(x):= \sum_{j_1=1}^n L_{j_1}(x)
\end{align*}
\end{definition}

The goal of gradient descent and stochastic gradient descent is starting from $x_0$ running iterative method for $T$ iterations and find a $x_T$ such that $L(x_T)$ is close to $L(x_*)$ in a certain sense, where $x_*=\min_{x} L(x)$.
\begin{definition}[Gradient descent]
For each iteration $t$, we update 
\begin{align*}
    x_{t+1} = x_{t} - \eta \cdot ( \nabla L(x) )|_{x= x_t}
\end{align*}
where $\eta > 0$ is the learning rate and $\nabla L(x) = \sum_{j_1=1}^n \nabla L_{j_1}(x)$ is the gradient of Loss function $L$.
\end{definition}

\begin{definition}[Stochastic gradient descent]
For each iteration $t$, we sample a set $B_t \subset [n]$, we update
\begin{align*}
    x_{t+1} = x_t - \eta \cdot \sum_{j_1 \in B_t} ( \nabla L_{j_1}(x) )|_{x = x_t}
\end{align*}
where $\eta$ is the learning rate.
\end{definition}

\subsection{Basic Equivalence}
\label{sub:gradient:eqivalence}
\Zhao{It's better to move this subsection to appendix, this calculation is not so important.}
Now, we introduce a basic equivalence. 
 
\begin{claim}
If the following conditions hold 
\begin{itemize}
    \item Let $b \in \R^{n^2}$ denote the vectorization of $B \in \R^{n \times n}$, i.e., $b = \vect(B)$
\end{itemize}
Then, we have
\begin{itemize}
\item Part 1.
\begin{align*}
\vect( \underbrace{ A_1 }_{n \times d} \underbrace{ X }_{d \times d} \underbrace{ A_2^\top }_{d \times n} ) = \underbrace{ ( A_1 \otimes A_2) }_{n^2 \times d^2} \underbrace{ \vect(X) }_{d^2 \times 1}
\end{align*}
\item Part 2. $\min_{X \in \R^{d \times d}} \| A_1 X A_2 - B \|_F^2$ is equivalent to $\min_{x \in \R^{d^2}} \| (A_1 \otimes A_2) x - b \|_2^2$.
\item Part 3. $\min_{X \in \R^{d \times d}} \| \exp( A_1 X A_2 ) - B \|_F^2$ is equivalent to $\min_{x \in \R^{d^2}} \| \exp( (A_1 \otimes A_2^\top ) x ) - b \|_2^2$.
\item Part 4. $\min_{X \in \R^{d \times d}} \| D(X)^{-1} \exp( A_1 X A_2^\top ) - B \|_F^2$ is equivalent to $\min_{x \in \R^{d^2}} \| D(x)^{-1} \exp( (A_1 \otimes A_2) x ) - b \|_2^2$.
\begin{itemize}
    \item The diagonal matrix $D(X) \in \R^{n \times n}$ is defined as $D(X) := \diag( \exp(A_1 X A_2^\top) {\bf 1}_n )$
    \item The diagonal matrix $D(x) \in \R^{n^2 \times n^2}$ is be written as $ D(x)= D(X) \otimes I_n$.
\end{itemize}
\end{itemize}
\end{claim}

\begin{proof}

{\bf Proof of Part 4.}

For each $i_1,i_2$-th entry in $D(X)^{-1} \exp(A_1 X A_2^\top) $ is same as $(i_1-1) n + i_2$-th entry in $D(x)^{-1} \exp((A_1 \otimes A_2) x)$.

Similarly, for $B$ and $b$.

Since all entries are matching, thus the norms are matching.

\end{proof}

\subsection{Basic Derivatives}
\label{sub:gradient:derivatives}

Now, we compute the first-order derivatives.

\begin{lemma}\label{lem:basic_derivatives}
If the following conditions hold
\begin{itemize}
    \item Let $A_1, A_2 \in \R^{n \times d}$.
    \item Let $\mathsf{A} = A_1 \otimes A_2$ (recall Definition~\ref{def:kronecker_product}).
    \item Let $X \in \R^{d \times d}$. 
    \item Let $D(x)$ be defined as in Definition~\ref{def:dx}.
    \item Let $x$ be a vector in $\R^{d^2}$, satisfying $x = \vect(X)$.
\end{itemize}
Then, we can show
\begin{itemize}
\item Part 1. For each $i \in [d^2]$,
\begin{align*}
    \frac{\d  \mathsf{A} x}{\d x_i} = \A_{*,i}
\end{align*}
\item Part 2. For each $i \in [d^2]$,
\begin{align*}
    \frac{\d \exp( \mathsf{A} x)}{\d x_i} = \exp( \mathsf{A} x) \circ \A_{*,i}
\end{align*}
\item Part 3. For each $j_1 \in [n] $, for each $i \in [d^2]$,
\begin{align*}
    \frac{\d \A_{[j_1],*} x }{\d x_i} = \A_{[j_1],i}
\end{align*}
\item Part 4. For each $j_1 \in [n]$, for each $i \in [d^2]$,
\begin{align*}
    \frac{\d u(x)_{j_1} }{\d x_i} = u(x)_{j_1} \circ \A_{[j_1],i}
\end{align*}
\item Part 5. For each $j_1 \in [n]$, for each $i \in [d^2]$,
\begin{align*}
    \frac{\d \alpha(x)_{j_1}}{\d x} = \langle u(x)_{j_1} , \A_{[j_1], i} \rangle
\end{align*}
\item Part 6. For each $j_1 \in [n]$, for each $i\in [d^2]$,
\begin{align*}
    \frac{\d \alpha(x)_{i_1}^{-1} }{\d x_i} = - \alpha(x)_{j_1}^{-1} \cdot \langle f(x)_{j_1}, \A_{[j_1],i} \rangle
\end{align*}
\item Part 7. For each $j_1 \in [n]$, for each $i \in [d^2]$,
\begin{align*}
    \frac{\d f(x)_{j_1}}{ \d x_i} = f(x)_{j_1} \circ \A_{[j_1],i} - f(x)_{j_1} \cdot \langle f(x)_{j_1}, \A_{[j_1],i} \rangle.
\end{align*}
\item Part 8. For each $j_1 \in [n]$, for each $i \in [d^2]$,
\begin{align*}
    \frac{\d c(x)_{j_1}}{ \d x_i} = \frac{\d f(x)_{j_1}}{\d x_i}
\end{align*}
\item Part 9. For each $i \in [d^2]$,
\begin{align*}
    & ~ \frac{\d L_{\exp}(x)}{ \d x_i} \\
    = & ~ \sum_{j_1=1}^n (\langle c(x)_{j_1}, f(x)_{j_1} \circ \A_{[j_1],i} \rangle - \langle c(x)_{j_1}, f(x)_{j_1} \rangle \cdot \langle f(x)_{j_1}, \A_{[j_1],i} \rangle).
\end{align*}
\end{itemize}
\end{lemma}

\Zhao{We can put above lemma in first 7 pages, but for proofs of above lemma, we should definitely move to appendix.}\Yeqi{Done}
 

==> preli_short.tex <==
\section{Preliminary}
\label{sec:preli}

We introduce the notations in this section. 

\paragraph{Notations.}


Now, we introduce the notations related to the matrices. Let $A$ be an arbitrary element in $\R^{n \times d}$. Let $i \in [n]$ and $j \in [d]$. We use $A_{i, j}$ to denote the entry of $A$ located at the $i$-th row and $j$-th column. $A_{i, *}$ represents a vector in $\R^d$ satisfying $(A_{i, *})_j = A_{i, j}$. Similarly, $A_{*, j}$ represents a vector in $\R^n$ satisfying $(A_{*, j})_i = A_{i, j}$. $A^\top \in \R^{d \times n}$ represents the transpose of $A$. $\|A\|$ and $\|A\|_F$ represent the spectral norm and the Frobenius norm of $A$, respectively, where $\| A \| = \max_{x \in \R^d} \| A x \|_2 / \| x \|_2$ and $\|A\|_F := \sqrt{\sum_{i \in [n]} \sum_{j \in [d]} |A_{i, j}|^2}$. We define the Kronecker product, denoted by $\otimes$, to be a binary operation between two matrices. For matrix $A \in \R^{n_1 \times d_1}$ and a matrix $B \in \R^{n_2 \times d_2}$, we use $A\otimes B \in \R^{n_1 n_2 \times d_1 d_2}$ to denote a new matrix that $(i_1 - 1) n_2 + i_2$, $(j_1-1)d_2+j_2$-th entry is $A_{i_1,j_1} B_{i_2,j_2}$, where $i_1 \in [n_1], j_1 \in [d_1], i_2 \in [n_2], j_2 \in [d_2]$.


